DemoGen: Synthetic Demonstration Generation for Data-Efficient Visuomotor Policy Learning

Visuomotor policies have shown great promise in robotic manipulation but often require substantial amounts of human-collected data for effective performance. A key reason underlying the data demands is their limited spatial generalization capability, which necessitates extensive data collection across different object configurations. In this work, we present DemoGen, a low-cost, fully synthetic approach for automatic demonstration generation. Using only one human-collected demonstration per task, DemoGen generates spatially augmented demonstrations by adapting the demonstrated action trajectory to novel object configurations. Visual observations are synthesized by leveraging 3D point clouds as the modality and rearranging the subjects in the scene via 3D editing. Empirically, DemoGen significantly enhances policy performance across a diverse range of real-world manipulation tasks, showing its applicability even in challenging scenarios involving deformable objects, dexterous hand end-effectors, and bimanual platforms. Furthermore, DemoGen can be extended to enable additional out-of-distribution capabilities, including disturbance resistance and obstacle avoidance.

==> sections/7_discussion.tex <==
\section{Discussions}
as a data generation method, decoupled with the policy learning method. can also be applied to offline RL, VLA.

scale up with \method. the effects will be magnified

Q: if planning can solve the task, then why train IL policy? A: we use a closed-loop IL policy to distill the knowledge of TAMP. the strength of IL is emergent retry and replan according to observation and external disturbance.

Q: why not one source demo for all tasks? A: Due to visual mismatch, \method cannot solve all the tasks from only one source demo. empirically, we find the capability upper-bound of \method-generated demos from one source demo is to obtain the same performance as around 25 source demos. That is, the effects of \method is roughly to reduce the need for human collected demonstrations by around 25x. 

Q: can \method be used on tasks requiring very high precision? A: yes, but those tasks often require a large number of source demonstrations. so one source demo is not enough for \method to solve these tasks.


==> sections/8_limitation.tex <==
\section{Limitations}
segmented point cloud

do not work for highly clustered scenes

single-view, translation, not too far away, object mismatch, ee still but arm might change

orientation,  not support full-scale orientation. e.g., a 180 deg yaw rotation may rotate the an unreachable ee state for the robot. solve by collecting some stem orientations. or through equivariant learning

limited by the performance of 3D observation policy. For example, simple pointnet encoder in dp3 is sensitive to the size of the manipulated objects. it will overlook small parts in the scene.
Also, with more demos, \method works for ``anywhere'' on the table surface? depend on the performance of the policy. can they memorize all the configurations? 
future: edit on 3D and then project to 2D

fixed position, contact-rich problems. in-hand object reorientation using dexterous hands, or push-T with fixed target pose.

do not work for highly precise (mm-level) tasks 

both 3d editing and DP3 policy learning require relatively high-quality point clouds. L515 is good, but D435 or Zedd is not good enough.
